Algorithms and Hardness for Diameter in Dynamic Graphs

The diameter, radius and eccentricities are natural graph parameters. While these problems have been studied extensively, there are no known dynamic algorithms for them beyond the ones that follow from trivial recomputation after each update or from solving dynamic All-Pairs Shortest Paths (APSP), which is very computationally intensive. This is the situation for dynamic approximation algorithms as well, and even if only edge insertions or edge deletions need to be supported. This paper provides a comprehensive study of the dynamic approximation of Diameter, Radius and Eccentricities, providing both conditional lower bounds, and new algorithms whose bounds are optimal under popular hypotheses in fine-grained complexity. Some of the highlights include: - Under popular hardness hypotheses, there can be no significantly better fully dynamic approximation algorithms than recomputing the answer after each update, or maintaining full APSP. - Nearly optimal partially dynamic (incremental/decremental) algorithms can be achieved via efficient reductions to (incremental/decremental) maintenance of Single-Source Shortest Paths. For instance, a nearly $(3/2+\epsilon)$-approximation to Diameter in directed or undirected graphs can be maintained decrementally in total time $m^{1+o(1)}\sqrt{n}/\epsilon^2$. This nearly matches the static $3/2$-approximation algorithm for the problem that is known to be conditionally optimal.

==> decremental32.tex <==
\section{Decremental algorithms}



% \begin{theorem}\label{thm:dec} Suppose there is a decremental approximate SSSP algorithm $\mathcal{A}$ with amortized update time $T$ such that given $\delta>0$, it maintains for a given vertex $u$, an estimate $d'(u,v)$ for all $v$ such that $(1-\delta)d(u,v)\leq d'(u,v)\leq d(u,v)$. Then there is a Las Vegas randomized algorithm for decremental diameter with total time $\tilde{O}(m\sqrt{n}T$) with high probability such that given any constant $\epsilon>0$ and a graph subject to edge deletions maintains an estimate $\hat{D}$ such that $(2/3)(1-\eps)D\leq \hat{D}\leq D$, where $D$ is the true diameter of the current graph.
% \end{theorem}

In this section we give a nearly $3/2$-approximation for decremental diameter, a nearly $3/2$-approximation for decremental radius, and a nearly $5/3$-approximation for decremental eccentricities, given access to a black-box decremental approximate SSSP algorithm as specified in the preliminaries. 
%Our algorithm works for directed graphs if $\mathcal{A}_{inc}$ works for directed graphs.




\begin{theorem}\label{thm:dec} There is a Las Vegas randomized algorithm for decremental diameter in unweighted, directed graphs that given $\eps>0$, runs in total time $\tilde{O}(\max_{D_0\leq D'\leq D_f}\{T_{dec}(n,m,D')\frac{\sqrt{n}}{\eps}\})$ with high probability, and maintains an estimate $\hat{D}$ such that $\frac{2(1-\eps)}{3}D-1\leq \hat{D}\leq D$ where $D$ is the diameter of the current graph. 
\end{theorem}

% We get the following corollary by using cite alg as the algorithm $\mathcal{A}$.

% \begin{corollary}
% Then there is a Las Vegas randomized algorithm for decremental diameter with total time $\tilde{O}(m\sqrt{n}$) in expectation such that given a constant $\epsilon>0$ and an undirected graph subject to edge deletions maintains an estimate $\hat{D}$ such that $(2/3)(1-\eps)D\leq \hat{D}\leq D$, where $D$ is the true diameter of the current graph.
% \end{corollary}


%TODO: derandomize?

\begin{proof}[Proof of Theorem~\ref{thm:dec}]$ $

% \subsection{Algorithm}

% \subsubsection*{Initialization}
% We randomly sample a set $S$ of $\Theta(\sqrt{n}\log n)$ vertices so that with high probability, for every vertex $v$, at every point in time, $S$ hits the closest $\sqrt{n}$ vertices to $v$. 

% Throughout the entire execution of the algorithm, we run algorithm $\mathcal{A}$ from each vertex in $S$. Additionally, we maintain the approximate distance from $S$ to every vertex by adding a dummy vertex $x$ adjacent to every vertex in $S$ and running algorithm $\mathcal{A}$ from $x$. We note that all executions of algorithm $\mathcal{A}$, except for the one from $x$, are with respect to the graph without $x$.

% BEGIN
\subsection{Algorithm}
Let $\delta=\eps/3$. Throughout the algorithm we will run in-$\mathcal{A}_{dec}$ and out-$\mathcal{A}_{dec}$ from carefully chosen sets of vertices. For every instantiation of these algorithms, we use the parameter $\delta$.

\paragraph*{Initialization}
%Let $\alpha$ be such that $ D'= \Theta(n^{1-2\alpha})$.
We randomly sample a set $S$ of size $\Theta(\sqrt{n}\log^2 n)$ so that with high probability, for every vertex $v$, after every update, $S$ hits $N_{out}(v,\sqrt{n})$.

Throughout the entire execution of the algorithm, we run in-$\mathcal{A}_{dec}$ from every vertex in $S$. Additionally, we maintain the approximate distance $d'(v,S)$ from every vertex $v$ to $S$ as described in the preliminaries.
% the approximate distance every vertex to $S$ by adding a dummy vertex $x$ with an edge from every vertex in $S$ to $x$ and running in-$\mathcal{A}$ from $x$. (We note that for all other purposes, $x$ is not included in the graph.) 
%Let $W$ be the dynamically changing set of vertices $v$ that satisfy $d'(v,S)> D'/3$.

\paragraph*{Phases}
The algorithm runs in phases. The first phase begins right after initialization. At the beginning of each phase, we let $w$ be the vertex that maximizes $d'(w,S)$.

%If $w$ is estimated to be of distance at most $D(\frac{(1-\delta)^2}{3})$ from some vertex in $S$, the algorithm description is done. Otherwise, we do the following. 
Throughout the phase, we run out-$\mathcal{A}_{dec}$ from $w$. We also run in-$\mathcal{A}_{dec}$ from every vertex in $B_{out}^<(w, d'(w,S))$. We note that since we are in the decremental setting, no vertex can join $B_{out}^<(w, d'(w,S))$.
% If at most $\sqrt{n}$ vertices are estimated by $\mathcal{A}$ to be of distance at most $D(\frac{(1-\delta)^2}{3})$ from $w$, then 
%  We also run in-$\mathcal{A}_{dec}$ from a subset $S'\subseteq B_{out}^<(w, d'(w,S))$ defined as follows. We independently add each vertex in $B_{out}^<(w, d'(w,S))$ to $S'$ with probability $\min\{1,\frac{\log^2 n}{\delta  d'(w,S)}\}$; additionally, whenever a vertex $u$ joins $B_{out}^<(w, d'(w,S))$ we add $u$ to $S'$ with probability $\min\{1,\frac{\log^2 n}{\delta  d'(w,S)}\}$.
 
 The beginning of a new phase is triggered when $d'(w,S)$ no longer approximates the largest distance from any vertex to $S$. More specifically, the beginning of a new phase is triggered when $d'(w,S)\leq (1-\delta)\max_{v\in V}(d'(v,S))$.

% We note that since we are in the decremental setting, the set of vertices of distance at most $D(\frac{(1-\delta)^2}{3})$ from $w$ cannot grow throughout the phase. 

\paragraph*{Reinitialization}

If at any point during the execution of the algorithm, $|B_{out}^<(w, d'(w,S))|> \sqrt{n}$, we reinitialize the entire algorithm. We will show in the analysis that with high probability we never reinitialize the algorithm.

% \begin{itemize}
%     \item $|B_{out}^<(w, d'(w,S))|> n^{1-\alpha}$
%     \item $|S'|> \frac{n^{1-\alpha}\log^4 n}{\delta  d'(w,S)}$
%     \item there is a vertex $v\in B_{out}^<(w, d'(w,S))$ such that $d'(v,S')>\delta  d'(w,S)$.
% \end{itemize}

\paragraph*{Query}

Following each update, the return value $\hat{D}$ is the maximum distance estimate found over all instantiations of out-$\mathcal{A}_{dec}$ and in-$\mathcal{A}_{dec}$. That is, $\hat{D}=\max\{\max_{v\in V}d'(w,v),\max_{v\in V,s\in S\cup S'}d'(v,s)\}$.



% Apply (1+\delta)-appx SSSP on each v in W and each s in S.

\subsection{Analysis}

\subsubsection*{Correctness}
% The proof of correctness is similar to that of the analogous static algorithm of  ref. The difference is that we have two additional sources of error: the algorithm $\mathcal{A}$ is an approximation and $w$ is an approximation of the farthest vertex from $S$.



The return value $ \hat{D}$ is $d'(u,v)$ for some $u,v$, so $ \hat{D}\leq D$. It remains to show that $\frac{2(1-\eps)}{3}D'-\frac{2}{3}\leq  \hat{D}$.

%Let $d'(u,v)$ be the distance from $u$ to $v$ as estimated by $\mathcal{A}$. 

Let $s^*$ and $t^*$ be the true diameter endpoints.

\noindent{\bf Case 1: There exists a vertex $s\in S$ such that $d'(s^*,s)\leq \frac{D}{3}$.} Then $d(s^*,s)\leq D(\frac{1}{3(1-\delta)})$. Then by the triangle inequality, $d(s,t^*)\geq D(1-\frac{1}{3(1-\delta)})$, so $\hat{D}\geq d'(s,t^*)\geq D(1-\delta)(1-\frac{1}{3(1-\delta)})=D(\frac{2}{3}-\delta)$.



\noindent{\bf Case 2: For all $s\in S$, $d'(s^*,s)> \frac{D}{3}$.} If $d'(w,t^*)\geq \frac{2 D}{3}$, then we are done. So suppose otherwise; that is, suppose $d'(w,t^*)< \frac{2 D}{3}$ so $d(w,t^*)< D(\frac{2}{3(1-\delta)})$. 


Consider the shortest path from $w$ to $t^*$. Let $q$ be the vertex on this path at distance $\lfloor D(\frac{(1-\delta)}{3})\rfloor\geq D(\frac{(1-\delta)}{3})-1$ from $w$. So, $d(s^*,q)\leq D(\frac{2}{3(1-\delta)}-\frac{(1-\delta)}{3})+1$. Thus, $d(q,t^*)\geq  D(1-\frac{2}{3(1-\delta)}+\frac{(1-\delta)}{3})-1$. So, $d'(q,t^*)\geq D(1-\delta)(1-\frac{2}{3(1-\delta)}+\frac{(1-\delta)}{3})-1=D(\frac{1}{3}-\delta+\frac{(1-\delta)^2}{3})-1$.

Since we are in case 2, $d'(w,S)>D(\frac{1-\delta}{3})$ as otherwise the beginning of a new phase would have been triggered. Thus, $q\in B_{out}(w, d'(w,S))$, so $\hat{D}\geq d'(q,t^*)$.


% Let $q$ be the vertex on this path at distance $\lfloor\frac{ D(1-\delta)}{3}\rfloor$ from $w$. So $d(q,t^*)<  D\frac{2}{3(1-\delta)}-\lfloor\frac{ D(1-\delta)}{3}\rfloor\leq  D(\frac{2}{3(1-\delta)}-\frac{1-\delta}{3})+1$. By the triangle inequality, $d(s*,q)$


% Since we are in case 2, $d'(w,S)>D(\frac{1-\delta}{3})$ as otherwise the beginning of a new phase would have been triggered. Thus, $q\in B_{out}(w, d'(w,S))$, so $d'(S',q)\leq\delta d'(w,S)$ or else we would have reinitialized the algorithm. Then, from the preliminaries $d(S',q)\leq\frac{\delta d'(w,S)}{1-2\delta}$. Let $q'\in S'$ be a vertex with $d(q',q)\leq\frac{\delta d'(w,S)}{1-2\delta}$.


% By the triangle inequality, $d(q',t^*)\leq d(q',q)+d(q,t^*)\leq  D(\frac{\delta}{1-2\delta}+\frac{2}{3(1-\delta)}-\frac{1}{3})+\frac{2}{3}$. By the triangle inequality, $d(s^*,q')\geq D- D(\frac{\delta}{1-2\delta}+\frac{2}{3(1-\delta)}-\frac{1}{3})-\frac{2}{3}\geq  D(\frac{4}{3}-\frac{\delta}{1-2\delta}-\frac{2}{3(1-\delta)})-\frac{2}{3}$. Thus, $\hat{D}\geq d'(s^*,q')\geq D(1-\delta)(\frac{4}{3}-\frac{\delta}{1-2\delta}-\frac{2}{3(1-\delta)})-\frac{2}{3})= D(\frac{4(1-\delta)}{3}-\frac{\delta(1-\delta)}{1-2\delta}-\frac{2}{3})-\frac{2}{3}$.


% Recall that $x$ is the dummy vertex adjacent to all vertices in $S$, so $d'(x,s)>\frac{D}{3}+1$. Thus, we have $d'(x,w)> D(\frac{1-\delta}{3})+1$, as otherwise a new phase would have been triggered. Since $d'(x,w)$ is an underestimate for $d(x,w)$, $d(x,w)> D(\frac{1-\delta}{3})+1$. Thus, for all $s\in S$, $d(s,w)> D(\frac{1-\delta}{3})$. Thus, $d'(s,w)>D(\frac{(1-\delta)^2}{3})$. Therefore, we run algorithm $\mathcal{A}$ from all vertices of distance at most $d'(s,w)>D(\frac{(1-\delta)^2}{3})$ from $w$.

% If $d'(w,s^*)\geq D(\frac{2}{3})$, then we are done. So suppose otherwise; that is, suppose $d'(w,s^*)< D(\frac{2}{3})$ so $d(w,s^*)<D(\frac{2}{3(1-\delta)})$. We run algorithm $\mathcal{A}$ from the node $q$ on this path at distance $D(\frac{(1-\delta)^2}{3})$ from $w$. Since $d(w,s^*)<D(\frac{2}{3(1-\delta)})$, we have $d(q,s^*)<D(\frac{2}{3(1-\delta)}-\frac{(1-\delta)^2}{3})$. Thus, $d(q,t^*)\geq  D(1-\frac{2}{3(1-\delta)}+\frac{(1-\delta)^2}{3})$. Thus, $d'(q,t^*)\geq D(1-\delta)(1-\frac{2}{3(1-\delta)}+\frac{(1-\delta)^2}{3})=D(\frac{1}{3}-\delta+\frac{(1-\delta)^3}{3})$.

Setting $\delta=\eps/3$ completes the proof of correctness.



% \noindent{\bf Case 1: $s^*\not\in W$.} Let $s\in S$ be such that $d'(s^*,s)\leq \frac{ D'}{3}$. Then $d(s^*,s)\leq D'(\frac{1}{3(1-\delta)})$. Then by the triangle inequality, $d(s,t^*)\geq D- D'(\frac{1}{3(1-\delta)})\geq  D'(1-\frac{1}{3(1-\delta)})$. Thus, $\hat{D}\geq d'(s,t^*)\geq  D'(1-\delta)(1-\frac{1}{3(1-\delta)})= D'(\frac{2}{3}-\delta$).

% \noindent{\bf Case 2: $s^*\in W$.} If $d'(w,t^*)\geq \frac{2 D'}{3}$, then we are done. So suppose otherwise; that is, suppose $d'(w,t^*)< \frac{2 D'}{3}$ so $d(w,t^*)< D'\frac{2}{3(1-\delta)}$. 

% Consider the shortest path from $w$ to $t^*$. Let $q$ be the vertex on this path at distance $\lfloor\frac{ D'}{3}\rfloor$ from $w$. So $d(q,t^*)<  D'\frac{2}{3(1-\delta)}-\lfloor\frac{ D'}{3}\rfloor\leq  D'(\frac{2}{3(1-\delta)}-\frac{1}{3})+\frac{2}{3}$. We know that $q\in B_{out}(w, \frac{ D'}{3})$, so $d'(S',q)\leq\delta D'$ or else we would have reinitialized the algorithm. Thus, from the preliminaries $d(S',q)\leq\frac{\delta D'}{1-2\delta}$. Let $q'\in S'$ be a vertex with $d(q',q)\leq\frac{\delta D'}{1-2\delta}$.


% By the triangle inequality, $d(q',t^*)\leq d(q',q)+d(q,t^*)\leq  D'(\frac{\delta}{1-2\delta}+\frac{2}{3(1-\delta)}-\frac{1}{3})+\frac{2}{3}$. By the triangle inequality, $d(s^*,q')\geq D- D'(\frac{\delta}{1-2\delta}+\frac{2}{3(1-\delta)}-\frac{1}{3})-\frac{2}{3}\geq  D'(\frac{4}{3}-\frac{\delta}{1-2\delta}-\frac{2}{3(1-\delta)})-\frac{2}{3}$. Thus, $\hat{D}\geq d'(s^*,q')\geq D'(1-\delta)(\frac{4}{3}-\frac{\delta}{1-2\delta}-\frac{2}{3(1-\delta)})-\frac{2}{3})= D'(\frac{4(1-\delta)}{3}-\frac{\delta(1-\delta)}{1-2\delta}-\frac{2}{3})-\frac{2}{3}$.



\paragraph*{Running time}

%  \item $|B_{out}^<(w, d'(w,S))|> n^{1-\alpha}$
%     \item $|S'|> \frac{n^{1-\alpha}\log^4 n}{\delta  d'(w,S)}$
%     \item there is a vertex $v\in B_{out}^<(w, d'(w,S))$ such that $d'(v,S')>\delta  d'(w,S)$.

\subparagraph{Reinitialization}
We will argue that with high probability, we never reinitialize the algorithm. The algorithm is reinitialized if $|B_{out}^<(w, d'(w,S))|> \sqrt{n}$. 
Recall that with high probability, for every vertex $v$, after every update, $S$ hits $N_{out}(v,\sqrt{n})$. 
%By the definition of $W$, $ D'/3<d'(w,S)\leq d(w,S)$.
Since $B_{out}^<(w, d'(w,S))$ contains no vertices in $S$, with high probability $B_{out}^<(w, d'(w,S))$ does not contain $N_{out}(v,\sqrt{n})$. That is, with high probability, $B_{out}^<(w, d'(w,S))< \sqrt{n}$.

% Another event that triggers reinitialization is if
% $|S'|> \frac{n^{1-\alpha}\log^4 n}{\delta  d'(w,S)}$. $|S'|$ is a random variable drawn from a binomial distribution with  $p=\frac{\log^2 n}{\delta d'(w,S)}$ and expected value $\frac{|B_{out}^<(w, d'(w,S))|\log^2 n}{\delta d'(w,S)}$. We know that $|B_{out}^<(w, d'(w,S))|\leq n^{1-\alpha}$ or else we would have reinitialized the algorithm due to the above event. Thus, $|S'|\leq  \frac{n^{1-\alpha}\log^4 n}{\delta  d'(w,S)}$ with high probability.

% The last event that triggers reinitialization is if there is a vertex $v\in B_{out}^<(w, d'(w,S))$ such that $d'(v,S')>\delta  d'(w,S)$.
% The expected size of $S'$ is $\frac{|B_{out}^<(w, d'(w,S))|\log^2 n}{\delta d'(w,S)}$. Thus, with high probability, for all vertices $v\in B_{out}^<(w, d'(w,S)$, after every update, $S'$ hits a vertex of distance at most $\delta d'(w,S)$ to $v$.

% We have shown that each of the three events that trigger reinitialization do not occur with high probability (probability at least $1-1/n^c$ for all constants $c$). Thus, with high probability we never reinitialize the algorithm.


\subsubsection*{Update time}

We will calculate the total number $k$ of vertices that we ever run out-$\mathcal{A}_{dec}$ or in-$\mathcal{A}_{dec}$ from. Then the total update time is $O(\max_{D_0\leq D'\leq D_f}T_{dec}(n,m,D')k)$ with high probability. 

In the initialization step, we initialize algorithm out-$\mathcal{A}_{dec}$ from all $\tilde{O}(\sqrt{n})$ vertices in $S$ as well as a dummy vertex. 

% We reinitialize the algorithm if $w$ is estimated by $\mathcal{A}$ to be of distance more than $\frac{D(1-\delta)^2}{3}$ from all vertices in $S$ and there are more than $\sqrt{n}$ vertices estimated to be of distance at most $\frac{D(1-\delta)^2}{3}$ from $w$. Recall that with high probability, at every point in time, $S$ hits the closest $\sqrt{n}$ vertices to $w$. Therefore, with high probability we never reinitialize the algorithm.

In each phase, we run algorithm $\mathcal{A}$ from $w$ as well as all the at most $\sqrt{n}$ vertices in $B_{out}^<(w, d'(w,S))$. 
%Note that all such vertices are in reality of distance at most $\frac{\tilde{D}}{3}$ from $w$. Since $x\in X$, $w$ is estimated to be of distance more than $\tilde{D}/3$ from $S$, so $w$ is truly of distance more than $\tilde{D}/3$ from $S$. Since $S$ hits the closest $\sqrt{n}$ vertices to $v$, there are only $\sqrt{n}$ vertices of distance at most $\tilde{D}/3$ from $w$, and thus there are only $\sqrt{n}$ vertices estimated to be of distance at most $\frac{\tilde{D}(1-\delta)}{3}$ from $w$. 
Thus, $k$ is at most $\sqrt{n}$ times the number of phases.

Now, we calculate the number of phases. Recall that the beginning of a new phase is triggered when $d'(w,S)\leq (1-\delta)\max_{v\in V}(d'(v,S))$. Since we are in the decremental setting, distances cannot decrease, so this inequality can only be satisfied as a result of an increase in $\max_{v\in V}d'(v,S)$. This value can be at most $n$, so the number of phases is $O(\log_{\frac{1}{1-\delta}}n)=\tilde{O}(\frac{1}{\eps})$.

Putting everything together, $k=\tilde{O}(\sqrt{n}/\eps)$, so the total update time is $\tilde{O}(\max_{D_0\leq D'\leq D_f}\{T_{dec}(n,m,D')\frac{\sqrt{n}}{\eps}\})$.

\end{proof}

% Statement:

% Let G=(V,E) be an undirected unweighted graph.  Let eps > 0. There is an algorithm that maintains (3+eps)/2 approximation to diameter in G in O(1/eps m^(1+o(1) sqrt(n) ) total time.

% Algorithm:

% Let eps > 0, delta > 0.

% The algorithm is divided to phases. At the beginning of each phase we execute BeginPhase procedure (to be followed).

% Initialization Procedure:

% Choose a set S of expected size O(sqrt(n)) such that w.h.p. S hits all sqrt(n) closest vertices for each v in V over all m=O(n^2) versions of the graph (per each update)

% BeginPhase Procedure:

% Let d_S(v) be the distance from v to the closest vertex in S.

% Apply the static algorithm: 
% Compute BFS for each s in S. Compute for each v in V, d_S(v) (this can be done on O(m) time by adding dummy vertex connected to all vertices... etc.).
% Let w be a vertex such that w = argmax {d_S(v)} (for each v in V).
% Let W be the closest sqrt(n) vertices to w. 

% Apply (1+\delta)-appx SSSP on each v in W and each s in S.

% Query: 

% return max{tilde(e(s))}_{s in (S cup W)} / (1+ delta) 

% Update: 

% Let e(v) be the eccentric of v. Similarly \tilde(e(v)) is the (1+delta) approximated eccentric of v maintained by the SSSP (1+delta) approximation.

% If d_S(w) <= max{tilde(e(s))}_{s in S} / (1+eps) invoke BeginPhase
% Otherwise update all (1+\delta)-appx SSSP

% Time Analysis:

% Computing S in the initialization step takes O(n) time. The time BeginPhase is the time for the static algorithm, which takes O( m sqrt(n) ). We also maintain (1+\delta)-appx SSSP due to Henzinger et al which totally takes O(m^{1+o(1)}). Since we apply it on O(sqrt(n)) vertices at most, the total time to maintain all SSSP for a phase is O(sqrt(n) m^{1+o(1)}). Since diameter can increase by a factor of (1+eps) only log_{1+eps}(n) times, BeginPhase will be invoked at most O(1/eps) times, so the total time for maintaining (1+delta)-appx SSSP overall is O(1/ eps sqrt(n) m^{1+o(1)})

% Note: the value max{tilde(e(s))}_{s in S} can be updated during the updates of the SSSP (so it is subsumed in the overall time)

% Accuracy Analysis:

% At the beginning of each phase we have 3/2 approximation. We need to show that after each update we have (3/2+eps) approximation.
% Let Dnew be the current diameter and let a and b its endpoints . 
% Denote d = d_S(w), d1 = max{tilde(e(s))}_{s in S}, d2 = max{e(s)}_{s in S}.

% Notice we always return approximation that is smaller than diameter since we divide by (1 + delta).

% If there is s in S such that e(s) >= 2/3 Dnew, we are done since since tilde(e(s)) >= 2/3(1+delta) Dnew.

% Otherwise, WLOG, d_S(a) < 2/3 Dnew. It follows that d_S(b) > Dnew / 3. Therefore, we get:
% Dnew / 3 < d_S(b) <= d2 <= d1 <= d(1+eps).
% So we have d > Dnew / 3 (1+eps)

% If e(w) >= 2/3 Dnew, we are done since since tilde(e(w)) >= 2/3(1+delta) Dnew. 

% Otherwise e(w) >= 2/3 Dnew, and in particular d(w,a) <= 2/3 Dnew. 
% Since there is an s in W, there must be a vertex x in W such that x on the shortest path from w to a and d(s,x) >= Dnew / 3 (1+eps). Therefore, d(x,a) = (1+2eps)/3(1+eps)Dnew and it follows that d(x,b) >= (2+eps)/3(1+eps)Dnew >= 2/3(1+eps)Dnew.
% We return therefore 2/3(1+eps)(1+delta)Dnew. By selecting eps' small enough we get 2/3(1+eps')Dnew.

\subsection{Radius}
\begin{theorem}\label{thm:decrad} There is a Las Vegas randomized algorithm for incremental radius in unweighted, undirected graphs that given $\eps>0$ runs in total time \\$\tilde{O}(\max_{R_0\leq R'\leq R_f}\{T_{dec}(n,m,R')\frac{\sqrt{n}}{\eps}\})$ with high probability, and maintains an estimate $\hat{R}$ such that $R\leq \hat{R}\leq \frac{3(1+\eps)}{2}R+1$ where $R$ is the radius of the current graph.
\end{theorem}

The algorithm is identical to the algorithm of Theorem~\ref{thm:dec} except all instantiations of in-$\mathcal{A}_{dec}$ and out-$\mathcal{A}_{dec}$ are replaced by the corresponding algorithm for undirected graphs, and the return value is different. The return value $\hat{R}$ is the minimum eccentricity estimate found; that is, $\hat{R}=\min_{s\in S\cup \{w\}}\max_{v\in V}d'(v,s)\}$.

The analysis of correctness follows.

Let $c^*$ be the true center of the graph. For all $s\in S\cup S'\cup \{w\}$, let $\varepsilon'(s)$ be the estimated eccentricity $\max_{v\in V}d'(s,v)$.

The return value $ \hat{R}$ is $\varepsilon'(v)$ for some $v$, so $R\leq \hat{R}$. It remains to show that $\hat{R}\leq \frac{3(1+\eps)}{2}R+1$.


\noindent{\bf Case 1: there exists $s\in S$ such that $d'(c^*,s)\leq \frac{ R}{2}$.} Then $d(c^*,s)\leq R(\frac{1}{2(1-\delta)})$. Then by the triangle inequality, $\varepsilon(s)\leq R(\frac{1}{2(1-\delta)})+R\leq  R(\frac{1}{2(1-\delta)}+1)$. So $\hat{R}\leq \varepsilon'(s)\leq R(\frac{1}{2(1-\delta)}+1)$.

\noindent{\bf Case 2: there does not exist $s\in S$ such that $d'(c^*,s)\leq \frac{ R}{2}$.} 
 Consider the shortest path from $w$ to $c^*$. Let $q$ be the vertex on this path at distance $\lfloor\frac{ R(1-\delta)}{2}\rfloor$ from $w$. So $d(q,c^*)\leq \lceil\frac{R(1-\delta)}{2}\rceil\leq \frac{R(1-\delta)}{2}+1$. 
% We know that $q\in B_{out}^\leq(w, \frac{ R}{2})$, so $d'(S',q)\leq\delta R'$ or else we would have reinitialized the algorithm. Thus, from the preliminaries $d(S',q)\leq\frac{\delta R'}{1-2\delta}$. Let $q'\in S'$ be a vertex with $d(q',q)\leq\frac{\delta R'}{1-2\delta}$.


% By the triangle inequality, $d(q',c^*)\leq d(q',q)+d(q,c^*)\leq  R'(\frac{\delta }{1-2\delta}+\frac{1}{2})+\frac{1}{2}$. 

By the triangle inequality, $\varepsilon(q)\leq R(1+\frac{(1-\delta)}{2})+1$.
Since we are in case 2, $d'(w,S)>R(\frac{1-\delta}{2})$ as otherwise the beginning of a new phase would have been triggered. Thus, $q\in B_{out}(w, d'(w,S))$, so $\hat{R}\leq \varepsilon'(q)\leq \varepsilon(q)$.

Setting $\delta= \eps/3$ completes the proof of correctness.


\subsection{Eccentricities}

\begin{theorem}\label{thm:incredecc} There is a Las Vegas randomized algorithm against an oblivious adversary for decremental eccentricities in unweighted, undirected graphs that given $\eps$ with $0<\eps<0.45$ runs in total time $\tilde{O}(\max_{D_0\leq D'\leq D_f}\{T_{dec}(n,m,D')\frac{\sqrt{n}}{\eps}\})$ with high probability, and for all $v\in V$ maintains an estimate $\hat{\varepsilon}(v)$ such that $\frac{3(1-\eps)}{5}\varepsilon(v)-1\leq \hat{\varepsilon}(v)\leq \varepsilon(v)$ where $\varepsilon(v)$ is the eccentricity of $v$ in the current graph.
\end{theorem}

The algorithm is identical to the algorithm of Theorem~\ref{thm:dec} except all instantiations of in-$\mathcal{A}_{dec}$ and out-$\mathcal{A}_{dec}$ are replaced by the corresponding algorithm for undirected graphs, and the return value is different. For all $s\in S\cup \{w\}$, let $\varepsilon'(s)$ be the estimated eccentricity $\max_{v\in V}d'(s,v)$. For all $v\in V$, the return value $\hat{\varepsilon}(v)=\max_{s\in S\cup \{w\}} \{d'(v,s),(1-\delta)\varepsilon'(s)-\frac{d'(v,s)}{1-\delta}\}$.

The analysis of correctness follows.

First we show that $\hat{\varepsilon}(v)\leq {\varepsilon}(v)$. If $\hat{\varepsilon}(v)=d'(v,s)$ for some $s$ then it is clear that $\hat{\varepsilon}(v)\leq \varepsilon(v)$. Otherwise, from the expression of the return value, for some $s$, $\hat{\varepsilon}(v)\leq(1-\delta)\varepsilon'(s)-\frac{d'(v,s)}{1-\delta}\leq \varepsilon(s)-d(v,s)\leq d(v,s')\leq \varepsilon(v)$. 

It remains to show that $\frac{3(1-\eps)}{5}\varepsilon(v)-1\leq \hat{\varepsilon}(v)$. Fix $v$.

\noindent{\bf Case 1. there exists $s\in S$ such that $d'(v',s)\leq 2\varepsilon(v)/5$.} Then $d(v',s)\leq\frac{2\varepsilon(v)}{5(1-\delta)}$. By the triangle inequality, $d(v,s)\geq \varepsilon(v)-d(v',s)\geq \varepsilon(v)(1-\frac{2}{5(1-\delta)})$. Then, $\varepsilon'(v)\geq d'(v,s)\geq \varepsilon(v)(1-\delta)(1-\frac{2}{5(1-\delta)})=\varepsilon(v)(3/5-\delta)$.

\noindent{\bf Case 2. for all $s\in S$, $d'(v',s)>2\varepsilon(v)/5$.} If $d'(w,v)\geq\frac{3\varepsilon(v)}{5}$, then we are done. So suppose otherwise; that is, suppose $d'(w,v)<\frac{3\varepsilon(v)}{5}$ so $d(w,v)<\frac{3\varepsilon(v)}{5(1-\delta)}$. 

Consider the shortest path from $w$ to $v$. Let $q$ be the vertex on this path at distance $\lfloor\frac{2\varepsilon(v)(1-\delta)}{5}\rfloor$ from $w$. So $d(q,v)<\frac{3\varepsilon(v)}{5(1-\delta)}-\lfloor\frac{2\varepsilon(v)(1-\delta)}{5}\rfloor\leq \frac{3\varepsilon(v)}{5(1-\delta)}-\frac{2\varepsilon(v)(1-\delta)}{5}+1$.


Since we are in case 2, $d'(w,S)>\frac{2\varepsilon(v)(1-\delta)}{5}$ as otherwise the beginning of a new phase would have been triggered. Thus, $q\in B_{out}(w, d'(w,S))$, so recall from the definition of the return value that  $\hat{\varepsilon}(v)\geq (1-\delta)\varepsilon'(q)-\frac{d'(v,q)}{1-\delta}\geq(1-\delta)^2\varepsilon(q)-\frac{d(v,q)}{1-\delta}$. 
By the triangle inequality, $\varepsilon(q)\geq d(q,v')\geq \varepsilon(v)-d(v,q)$. So,  $\hat{\varepsilon}(v)\geq (1-\delta)^2(\varepsilon(v)-d(v,q))-\frac{d(v,q)}{1-\delta}\geq (1-\delta)^2\varepsilon(v)-d(v,q)((1-\delta)^2+\frac{1}{1-\delta})$.

% By the triangle inequality, $d(x,v)\leq d(x,q)+d(q,v)\leq \frac{\delta E_j}{1-2\delta}+\frac{3\varepsilon(v)}{5(1-\delta)}-\frac{2E_j}{5}+\frac{4}{5}\leq \varepsilon(v)(\frac{\delta}{1-2\delta}+\frac{3}{5(1-\delta)}-\frac{2}{5})+\frac{4}{5}$. 

Combining the previous two paragraphs, we have $\hat{\varepsilon}(v)\geq\varepsilon(v)((1-\delta)^2- (\frac{3}{5(1-\delta)}-\frac{2(1-\delta)}{5})((1-\delta)^2+\frac{1}{1-\delta}))-1$.

One can verify that for all $\delta<0.05$, $((1-\delta)^2- (\frac{3}{5(1-\delta)}-\frac{2(1-\delta)}{5})((1-\delta)^2+\frac{1}{1-\delta}))\geq 3(1-9\delta)/5$. Thus we can set $\delta=\eps/9$ and obtain the result.

==> intro.tex <==

% Motivation take #1:
Demetrescu and Italiano~\cite{DemetrescuI04} obtained a fully dynamic APSP algorithm with an amortized update time of $\title{O}(n^2)$ and $O(1)$ query time. 

There are many important distance related parameters in graphs, such as \emph{vertex eccentricity} (the longest shortest path that contains the vertex),  graph \emph{diameter} (the maximum over all vertex eccentricities), \emph{radius} (the minimum over all vertex eccentricities). These parameters can be easily computed when all the distances are known. 

In many cases the analyzed dynamic graph is large that even enumerating all pairs of vertices is prohibitively expensive and therefore, maintaining all distances is essentially impossible. For graph parameters such as diameter and radius, the output is a single number; in principle looking at all pairs of vertices might not be necessary, and subquadratic time algorithms might exist. 
The question whether such fast dynamic algorithms exist  is interesting both from practical and theoretical perspectives.

% Related work: static diameter and radius
The research on dynamic algorithms is motivated by the goal of obtaining algorithms with an update time that is faster than the best static algorithm for the problem. 


There are certain restricted cases (such as APSP in unweighted graphs) in which the fastest known APSP algorithms run in subcubic time but use {\em Fast Matrix Multiplication\/} (FMM) and rely on impressive but highly impractical techniques~\cite{zwickbridge,Seidel95,v12,cw90,legallmult} and hence do not suit for dynamic problems. 
However, there are not any  static algorithms for diameter, radius and eccentricities that are  significantly faster than the APSP-based algorithm in general graphs.
Vassilevska W. and Williams~\cite{WilliamsW10} defined the notion of subcubic equivalence for dense graphs and asked whether one can show that the computation of some of these graph parameters is equivalent to the computation of APSP in dense graphs. 
No such subcubic equivalence to APSP is known for these parameters. 

In order to obtain some progress for theses problems natural relaxed variants were considered. A popular relaxation is to compute   \emph{approximation} of the parameter rather than its exact value.

% prevoius approx diameter results 

Aingworth et al.~\cite{ACIM99} obtained an algorithm that approximates the diameter $D$ of a directed unweighted graph  in $O(m\sqrt{n\log n}+ n^2\log n)$ time. The algorithm computes an estimate $\hat{D}$, such that $\lfloor 2/3 D \rfloor \leq \hat{D} \leq D$.
Roditty and V. Williams~\cite{RW13} presented an $\Ot(m\sqrt{n})$-time approximation algorithm to the diameter with the same  approximation as Aingworth \etal~\cite{ACIM99}.
For weighted graphs Chechik et al.~\cite{ch14} presented an algorithm that returns an estimate $\hat{D}$ for diameter $D$, such that $2/3 D \leq \hat{D} \leq D$ in time $\Ot(\min(m^{3/2},mn^{2/3}))$. 

% Lower bounds to lead to our upper bounds 

In this paper we show that it is very unlikely that fully dynamic algorithms with  truly subquadratic update time exist for these parameters, even if we relax the demand to exact result and allow approximations. 
In particular, we show for the diameter in  unweighted, undirected  graph there is no  $(3/2-\eps)$-approximation with truly subquadratic update time, assuming the SETH conjecture. 
For the  radius in unweighted, undirected we show that there is no  $(3/2-\eps)$-approximation with truly subquadratic update time under HS. 
For the  eccentricities in unweighted, undirected we show that there is no  $(5/3-\eps)$-approximation with truly subquadratic update time under SETH. 
All these bounds hold also even when the graph is sparse.  



Results to talk about: 

Decremental single source shortest path (SSSP) exact only Even and Shiloach. 

Decremental single source shortest path approximated  directed
and undirected. 

Incremental SSSP

The ES tree data structure~\cite{EvenS81} is a deterministic data structure for this setting in both directed and undirected, unweighted graphs. It gives exact distances and takes $O(n)$ amortized time per update.
In~\cite{HenzingerKNICALP13} another deterministic data is given for undirected, unweighted graphs. It maintains a $(1-\delta)$-approximation in amortized time $O(m^{2/3} ({\frac {n}{\eps^2 D}})^{1/3} \log n)$. Note that in sparse graphs this is faster than the ES tree when $D$ is ``close'' to $n$.




% Our techniques ideas:
% - describe static alg how we sample, find farthest away vertex w, then BFS from the closest sqrt{n} vertices to w. Still use initial sample, goal is to not have w change too often bc then need to reinitialize the algorithm from all those closest sqrt{n} to the new w. In the decremental setting, the idea is that the farthest vertex can only get farther. The key is that We show that when the farthest vertex gets much farther than the w that we chose, then the diameter must have increased, and the diameter can only increase by so much. For the incremental setting, it is more interesting because the farthest vertex and w get closer. So bad stuff is triggered when w gets closer. But if an edge is added between w an the set, that's bad and we need to choose a new w. This could happen over and over again. Solve by observing that we don't need w to be the actual farthest, just carefully defined sufficiently far and there could be a number of vertices that fit this criteria. Then using randomization against an oblivious adversary, we choose one sufficiently far vertex at random so that in expectation it takes a while for the adversary to find it (kind of), or adversary needs to pay to find it and make it close. The "sufficiently far" depends on the diameter itself so on top of this we perform a binary search for the diameter to get a proxy for D to carry our this stuff. For eccentricities it is less clear what sufficiently far means as we're trying to get all eccentricities. We try a bunch of different values simultaneously and show that for each eccentricity, at least one of the values works.  The first issue that we solve is the changing w and farthest and we do this differently in both the decremental and incremental settings. The second issue that we solve for decremntal directed and incremental both undirected and directed, the best known approximate SSSP alg is ES trees (not approximate). The running time is linearly dependent on the diameter. In the static setting, constant diameter is the "hard case". Whereas suddenly in the dynamic setting having a large diameter adds to the running time. There is a new challenge here that wasn't in other setting. To address this challenge, we do more precise subsampling since if there's a large diameter, we can afford to hit a vertex that is delta*D from the one that we really want to run BFS from, whereas if diam is constant then we can't sample vertex far away - it's useless.

% For lower bounds describe stages approach introduced in V/A paper and say that they just had that one 4/3 approx but we do more things with this approach to get improved lower bounds and trade-off ones. new constructions that get LB for just one eccentricity and thus SSSP. Stages in OV more generally applicable in getting trade-off e.g.
